A Geometric Approach to Problems in Optimization and Data Science

We give new results for problems in computational and statistical machine learning using tools from high-dimensional geometry and probability. We break up our treatment into two parts. In Part I, we focus on computational considerations in optimization. Specifically, we give new algorithms for approximating convex polytopes in a stream, sparsification and robust least squares regression, and dueling optimization. In Part II, we give new statistical guarantees for data science problems. In particular, we formulate a new model in which we analyze statistical properties of backdoor data poisoning attacks, and we study the robustness of graph clustering algorithms to ``helpful'' misspecification.

==> QueryComplexity/paper.tex <==
\chapter{Query complexity of certifying monotone functions \label{chapter:querycomplexity}}

==> SparsifyingNorms/maxnorm/results.tex <==
\def\arraystretch{1.3}
% \todo{there is $m$ vs $1/\epsilon$ tradeoff here I think, or is it being hidden in the per iteration computation of the methods? Either case clarify and point out.}
% \todo{I feel like it is not obvious that the per iteration complexity is comparable across these algorithms. Perhaps we can use the same base operation across methods, such as a single vector arithmetic operation, because iterations really have no meaning in this problem, only total computation does?}
\begin{table}[h]
\centering
\begin{tabular}{l c c} 
\toprule\toprule
\textbf{Algorithm}                                                                                                     & \textbf{Iteration Complexity}                                                                              & \textbf{Each Iteration}                     \\ \midrule\midrule
\makecell[l]{Subgradient descent}                                                                                           & \makecell[c]{$\frac{\norm{\xstar}_2 \max_{1 \le i \le m} \opnorm{\mA_{S_i}}}{\eps^{2}}$}                                   & \makecell[c]{Evaluate $\nabla f(\vx)$}                    \\ \midrule
\makecell[l]{Nesterov acceleration\\ on smoothened objective}                                                                 & \makecell[c]{$\frac{\norm{\xstar}_2 \left(\max_{1 \le i \le m} \opnorm{\mA_{S_i}}\right)^{1/2}}{\eps}$}                      & \makecell[c]{Evaluate $\nabla \ftilde_{\beta,\delta}(\vx)$} \\ \midrule
\makecell[l]{\cite{aakmrz22}}                                                                                               & \makecell[c]{$\frac{\norm{\xstar}_2 \max_{1 \le i \le m} \opnorm{\mA_{S_i}}}{\eps}$}                                       & \makecell[c]{Evaluate $\nabla \ftilde_{\beta,\delta}(\vx)$} \\ \midrule
\makecell[l]{Interior point with\\ log barrier \cite{boyd2004convex}}                                                         & \makecell[c]{$m^{1/2} \log\left(\frac{1}{\eps}\right)$}                                                                    & \makecell[c]{Linear system solve in $\mA^{\top}\mB\mA$}    \\ \midrule
\makecell[l]{Na\"ive application of \\ \cite{msbacon}}                                                                                          & \makecell[c]{$\frac{m^{1/3}}{\eps^{2/3}}$}                                                                                & \makecell[c]{Linear system solve in $\mA^{\top}\mB\mA$}    \\ \midrule
\makecell[l]{$\ell_{\infty}$ regression with\\ Lewis weights \cite{jls21}}                                                    & \makecell[c]{$\frac{\rank{\mA}^{1/3}}{\eps^{2/3}}$}                                                                       & \makecell[c]{Linear system solve in $\mA^{\top}\mD\mA$}    \\ \midrule
\makecell[l]{$\ell_{\infty}$ regression\\ with IPM \cite{ls19}}                                                               & \makecell[c]{$\rank{\mA}^{1/2} \log\left(\frac{1}{\eps}\right)$}                                                           & \makecell[c]{Linear system solve in $\mA^{\top}\mD\mA$}    \\ \midrule
\makecell[l]{\textbf{This chapter (\Cref{mainthm:fair_regression_iteration_complexity})}}                                                                                                    & \makecell[c]{$\frac{\min(\rank{\mA},m)^{1/3}}{\eps^{2/3}}$}                                                               & \makecell[c]{Linear system solve in $\mA^{\top}\mB\mA$}    \\ \bottomrule\bottomrule
\end{tabular}
\caption{Here, we list the complexities of algorithms for optimizing \eqref{eq:main_objective} or for $\ell_{\infty}$ regression, assuming $\opt=1$ (the first three guarantees are additive approximations) and ignoring $\mathrm{polylog}(n,m)$ terms. We write $\mD$ to be a diagonal matrix and $\mB$ to be a block-diagonal matrix where each block has size $(\abs{S_i} + o(1)) \times (\abs{S_i} + o(1))$. See the discussion in \cite[Section 1.2]{jls21} for why we focus on linear system solve complexities for the second-order methods. We remark that in the special case where $\abs{S_i}=1$, our algorithm exactly recovers that of \cite{jls21}.\label{table:compare}}
\end{table}

\subsubsection{Group distributionally robust linear regression}

Our first result is an algorithm for optimizing \eqref{eq:main_objective} up to the guarantee \eqref{eq:objective_approx} that overcomes all of the difficulties mentioned in the previous section. We state our guarantee in the following theorem.

\begin{mainthm}
\label{mainthm:fair_regression_iteration_complexity}
Let $\mA_{S_1},\dots,\mA_{S_m}$ be such that $\mA_{S_i} \in \R^{n_i \times d}$ and let $\vb_{S_1},\dots,\vb_{S_m}$ be such that $\vb_{S_i} \in \R^{\abs{S_i}}$. Let $\mA \in \R^{(\sum_{i=1}^m n_i) \times d}$ and $\vb \in \R^{\sum_{i=1}^m n_i}$ be formed by stacking the $\mA_{S_i}$ and $\vb_{S_i}$. Let $\eps > 0$. 

There exists an algorithm (\Cref{alg:fair_regression}) that returns $\xhat$ satisfying \eqref{eq:objective_approx} and runs in
\begin{align*}
    O\inparen{\frac{\min\inbraces{\mathsf{rank}(\mA),m}^{1/3}\inparen{\logv{\nfrac{n\log m}{\eps}}^{14/3}+\logv{m}}}{\eps^{2/3}}}
\end{align*}
linear system solves in matrices of the form $\mA^{\top}\mB\mA$, where $\mB$ is a block-diagonal matrix where each block has size $\abs{S_i} \times \abs{S_i}$.
\end{mainthm}

We compare the guarantee of \Cref{mainthm:fair_regression_iteration_complexity} against those of the other black-box methods that we are aware of in \Cref{table:compare}. From this, we see that unlike the mentioned first-order methods, our algorithm does not have any geometry-dependent terms. Additionally, our algorithm improves over the standard log-barrier IPM when the desired accuracy $\eps \ge m^{-1/4}$ -- this improvement is more pronounced when $m \gg \rank{\mA}$, which is the case in which the number of data sources is much larger than the dimension of the parameter vector $\vx$. Additionally, for $\eps \ge \rank{\mA}^{-1/4}$, our guarantee matches the best known guarantee for $\ell_{\infty}$ regression \cite{ls19,jls21}.

.\nnote{mention that this is the first result that gets closer to what we'd like to see for convex quadratic programs}

\subsubsection{Interpolating between average and robust losses}

Next, we introduce a parameter $p \in [2,\infty)$ and give a result for minimizing the family of objectives
\begin{align*}
    \inparen{\sum_{i=1}^m \norm{\mA_{S_i}\vx-\vb_{S_i}}_2^p}^{1/p}.
\end{align*}
Observe that choosing $p=2$ gives us a least-squares problem that is formed by stacking all the designs and responses, and $p=\infty$ recovers the problem \eqref{eq:main_objective}. Thus, varying $p$ between $2$ and $\infty$ and minimizing yields solutions that interpolate between the average and robust losses. It is natural to ask for the minimizer for some choice of $p \in (2,\infty)$ to smoothly trade off utility ($p=2$) and robustness ($p=\infty$). To this end, we give \Cref{mainthm:gp_regression_iteration_complexity}.

\begin{mainthm}
\label{mainthm:gp_regression_iteration_complexity}
Let $\mA,\vb,\eps$ be as defined in \Cref{mainthm:fair_regression_iteration_complexity}. 

There exists an algorithm that returns $\xhat$ for which
\begin{align*}
    \inparen{\sum_{i=1}^m \norm{\mA_{S_i}\xhat-\vb_{S_i}}_2^p}^{1/p} \le (1+\eps)\min_{\vx\in\R^d}\inparen{\sum_{i=1}^m \norm{\mA_{S_i}\vx-\vb_{S_i}}_2^p}^{1/p}.
\end{align*}
The algorithm runs in
\begin{align*}
    O\inparen{p^{20/3}\min\inbraces{\rank{\mA},m}^{\frac{p-2}{3p-2}}\logv{\frac{pd}{\eps}}^2}
\end{align*}
linear system solves in matrices of the form $\mA^{\top}\mB\mA$, where $\mB$ is a block-diagonal matrix whose blocks have size $\abs{S_i} \times \abs{S_i}$.
\end{mainthm}

In the proof of \Cref{mainthm:gp_regression_iteration_complexity}, we do not try too hard to optimize the exponent on $p$ or the logarithmic factors, as the main goal is to show that we can get an iteration complexity of the form $O(\mathsf{poly}(p,\logv{\frac{1}{\eps}})\min\inbraces{\rank{\mA},m}^{1/3})$. We suspect that some of these dependences, particularly the exponent in $p$, can be improved.

In the special case where $\abs{S_i}=1$ for all $i$ (and therefore the problem is $\ell_p$ regression for $p \ge 2$), the complexity promised by \Cref{mainthm:gp_regression_iteration_complexity} is comparable to that promised by \citet{jls21} for $\ell_p$ regression. The main difference is that the iteration complexity we give is unconditionally polynomial in $p$, whereas the comparable result from \cite{jls21} seems to require mild assumptions on the problem parameters (see the ``Discussion on numerical stability'' in Section 4). 


==> SparsifyingNorms/paper_1_app.tex <==
\section{Improved guarantees for sensitivity sampling}
\label{sec:sensitivity}

In this section, we give a self-contained analysis of another natural row sampling scheme -- sampling proportional to $\ell_p$ sensitivities. This appeared in the body in an earlier version of the manuscript, but it was pointed out to us by anonymous referees that the relation between sensitivities and Lewis weights was already established by \citet[Theorem 2.1]{cd21} (though it was not directly used for sampling). Nonetheless, we include it, partly because our proof of the relationship between sensitivities and Lewis weights is different from that of \cite{cd21} and is, in our opinion, simpler. We remark that a subsequent work by \citet{mo24_notus} shows that the dependence we obtain here is in fact tight.

\paragraph{Improved $\ell_p$ sensitivity sampling for $1 \le p < 2$.} We consider the problem of matrix row sampling proportional to $\ell_p$ sensitivity scores where $1 \le p \le 2$. See \Cref{defn:sensitivity}.

\begin{definition}[$\ell_p$ sensitivity {\cite[Section 1.3.1]{mmwy21}}]
\label{defn:sensitivity}
Let $\mA \in \R^{m \times d}$. The $\ell_p$ sensitivity of row $i$, denoted as $s_{i,p}(\mA)$, is
\begin{align*}
    s_{i,p}(\mA) \coloneqq \max_{\vx\in\R^d\setminus \inbraces{0}} \frac{\abs{\ip{\va_i,\vx}}^p}{\norm{\mA\vx}_{p}^p}.
\end{align*}
When $p$ and $\mA$ are clear from context, we omit them and simply write $s_i$ in place of $s_{i,p}(\mA)$.
\end{definition}

Essentially, $s_i$ gives an upper bound to the maximum possible relative contribution that the component $\abs{\ip{\va_i,\vx}}^p$ could make to the function $\norm{\mA\vx}_{p}^p$. 

Our main result in this setting is Theorem \ref{thm:main_sensitivity}.

\begin{restatable}[Sensitivity sampling for $1 \le p \le 2$]{mainthm}{sensitivity}
\label{thm:main_sensitivity}
Let $\cG = (\mA \in \R^{n \times d}, S_1,\dots,S_m, 1,\dots,1)$ where $\abs{S_1}=\dots=\abs{S_m}$. Let $p \ge 1$ (note that $n=m$ here).

For the probability distribution $\cD = \inparen{\rho_1,\dots,\rho_m}$ where $\rho_i \propto s_{i}$, if
\begin{align*}
    \mtilde &= \Omega\inparen{\logv{\nfrac{1}{\delta}}\vbrho \cdot\inparen{\sum_{i=1}^m s_i}d^{1-p/2}},
\end{align*}
and if we sample $\cM \sim \cD^{\mtilde}$, then, with probability $\ge 1-\delta$, we have:
\begin{align*}
    \text{for all } \vx \in \R^d,\quad (1-\eps)\norm{\mA\vx}_{p}^p \le \frac{1}{\mtilde}\sum_{i \in \cM} \frac{1}{\rho_i} \cdot \abs{\ip{\va_i,\vx}}^p \le (1+\eps)\norm{\mA\vx}_{p}^p
\end{align*}
\end{restatable}

To prove \Cref{thm:main_sensitivity}, we first need the following lower bounds on sensitivities. These were already proven in \cite[Theorem 2.1]{cd21}, but we believe our proof is more straightforward.

\begin{lemma}
\label{lemma:sens_lb}
Let $\vlambda$ denote Lewis's measure for $\mA$. For all $i \in [m]$, we have $\lambda_i \le s_i d^{-p/2}$.
\end{lemma}
\begin{proof}[Proof of \Cref{lemma:sens_lb}]
Let $\mW \coloneqq n\mLambda$. By monotonicity of $p$-norms under probability measures and the definition of the $s_i$, notice that we have for all $i \in [m]$ and all $\vx\in\R^d$ that
\begin{align*}
    \frac{\abs{\ip{\va_i,\vx}}}{s_i^{1/p}d^{1/p-1/2}} \le \frac{\norm{\mA\vx}_p}{d^{1/p-1/2}} \le \norm{\mW^{1/2-1/p}\mA\vx}_2.
\end{align*}
Next, recall that a standard (but fundamental) property of Lewis's measure is that it satisfies
\begin{align*}
    \max_{\vx\in\R^d\setminus\inbraces{0}} \frac{\abs{\ip{\va_i,\vx}}}{\norm{\mW^{1/2-1/p}\mA\vx}_2} = \tau_i(\mW^{1/2-1/p}\mA)^{1/2} \cdot w_i^{1/p-1/2} = w_i^{1/p}.
\end{align*}
This means that
\begin{align*}
    s_i^{1/p}d^{1/p-1/2} \ge w_i^{1/p},
\end{align*}
so taking the $p$th power of both sides yields $w_i \le s_i \cdot d^{1-p/2}$. Recalling the definition of $w_i$ concludes the proof of \Cref{lemma:sens_lb}.
\end{proof}

We are now ready to prove \Cref{thm:main_sensitivity}.

\begin{proof}[Proof of Theorem \ref{thm:main_sensitivity}]
Let $\mLambda$ be Lewis's measure on $[m]$, and recall the conclusion of \Cref{lemma:sens_lb}.

Next, in order to plug this into our framework, we observe that $\rho_i = s_i/(\sum_{j \le m} s_j)$. We now establish the overestimate
\begin{align*}
    d^{-p/2}\rho_i = \frac{d^{-p/2}s_i}{\sum_{j \le m} s_j} \ge \frac{\lambda_i}{\sum_{j \le m} s_j},
\end{align*}
and so after rearranging, we see that
\begin{align*}
    \inparen{d^{-p/2}\sum_{j \le m} s_j}\rho_i \ge \lambda_i.
\end{align*}
In particular, this means that we can set $H =  C\inparen{d^{-p/2}\sum_{j \le m} s_j}$ for some universal constant $C$ (as \cite[Theorem 1.6]{wy23_sens} shows that $\sum_{j \le m} s_j \gtrsim d^{p/2}$) and choose $\vlambda$ according to Lewis's measure. Then, since $H \ge 1$ and $\alpha_i^p = \lambda_i d^{p/2}$ (which in particular means that $\alpha_i^p/\norm{\valpha}_p^p = \lambda_i$), by \Cref{thm:concentration}, we get
\begin{align*}
    \mtilde \lesssim \vbrho\inparen{\sum_{i=1}^m s_i}d^{1-p/2},
\end{align*}
which completes the proof of \Cref{thm:main_sensitivity}.
\end{proof}

\paragraph{Discussion.} Arguably the most natural measure of row importance is when $\rho_i \propto s_i$ (recall \Cref{defn:sensitivity} for the definition of $s_i$). However, it is not known whether the sparsity of this instantiation of $\rho_i$ has $d$-dependence $d^{\max(1,p/2)}$. This is the optimal dependence on $d$ and is achieved by choosing the $\rho_i$ to be proportional to Lewis's measure. The previous best analysis for $\rho_i \propto s_i$ yielded a sparsity $\widetilde{O}(\eps^{-2}(\sum s_i)^{2/p})$ when $1 \le p \le 2$, due to \citet{wy23_sens}. To contrast this against our \Cref{thm:main_sensitivity}, we start by noting that by \cite[Theorem 1.6]{wy23_sens}, we have $\sum_{i\le m} s_i \gtrsim d^{p/2}$, so after raising both sides to the $2/p-1$-power and then multiplying both sides by $\sum_{i \le m} s_i$, we get
\begin{align*}
    \inparen{\sum_{i=1}^m s_i}^{2/p} \gtrsim \inparen{\sum_{i=1}^m s_i}d^{1-p/2}.
\end{align*}
Notice that the bound given by \citet{wy23_sens} occurs on the left and ours occurs on the right. In turn, this shows that our \Cref{thm:main_sensitivity} further sharpens the best-known analysis of row sampling by $\ell_p$ sensitivities when $1 \le p \le 2$. Furthermore, our worst-case guarantees improve over that given in \cite{wy23_sens} by a factor of $d^{2/p+p/2-2}$; in particular, when $p=1$, this amounts to an improvement of a factor of $d^{1/2}$.

For $p=2$, we note that $s_i = \tau_i$ where $\tau_i$ is the $i$th leverage score of $\mA$. Therefore, setting $\rho_i \propto s_{i,2}$ yields optimal sparsity bounds. Finally, a recent result due to \citet{pwz23} gives fast algorithms for estimating the $s_i$ in various parameter ranges.

==> intro_old.tex <==
\chapter{Introduction}

In the last few years, there has been a surge in the use of quantitatively based models across most application domains. Practitioners derive insights from an ever-growing trove of data. They subsequently use their findings to support their own research, build products, or anything in between. The field of \textit{algorithmic data science} addresses the natural algorithmic challenges that arise in any stage of this process. Here, the algorithmist's goal is to choose some subroutine from any aspect of the modern data science pipeline and either 1) build efficient algorithms with provable guarantees for this task, or 2) give an understanding of the fundamental limitations of various models of computation when applied to the task.

While the algorithmic toolkit for data science problems is growing, it is not clear how brittle known algorithmic guarantees are to the assumptions upon which they are proven. In many cases, these conditions are chosen to make the algorithmic problems mathematically tractable. An unfortunate consequence is that these conditions may not accurately reflect real-world scenarios. For example, in practice, the input dataset may be corrupted by malicious or ``inconvenient'' data. Conceivably, the output of an algorithm run using this unclean data may be very different from its output when given a clean input (i.e., one that satisfies the assumptions under which its original guarantees were derived). On the other hand, the input data may be clean but too unwieldy to practically work with. Perhaps our dataset has too many features (high dimensionality), or there may be too many observations to process all at once (big data). It is therefore important to build algorithmic solutions for these more realistic scenarios.

As a step towards designing more applicable algorithms, researchers have built new settings and models under which we can study classical algorithmic data science questions. We will explore problems in the following specific cases:
\begin{itemize}
    \item the \textit{malicious adversarial} setting, where an adversary is allowed to make harmful modifications to the input;
    \item the \textit{monotone adversarial} setting, which is a special case of the malicious adversarial model where the adversary's changes must be consistent with the original ground truth solution;
    \item the \textit{streaming} model, where the algorithm cannot store too much information about the input but is allowed to make a limited number of passes over the data;
    \item the \textit{coreset} model, where the algorithm is required output a weighted subsample of the original dataset while retaining certain statistics of the original dataset;
    \item the \textit{query} model, where the algorithm is allowed to read the input at various points but is not allowed to see it in its entirety.
\end{itemize}
We will also see some cases where part of the challenge is to design the correct assumptions to reflect a realistic input situation.

In light of this discussion, it will be helpful to keep the following guiding (and very informal) questions in mind throughout the rest of this thesis.

\begin{question}
How do we build input models or models of computation to either reflect input scenarios occurring in practice or to constrain algorithms in more applicable ways?
\end{question}

\begin{question}
Once we have designed such input assumptions or computational restrictions, can we actually build algorithms to apply in these settings?
\end{question}

The goal of this thesis is to give a better understanding of possible answers to the above questions. We will study several algorithmic problems with applications to data science in which the input is corrupted (\textit{adversarial input}) or cannot be accessed easily (\textit{restricted input access}). Although these problems are designed to answer very different questions, a key commonality is that they become far easier to solve (or, in some cases, outright trivial) when we replace the corrupted data with clean data or if we allow full access to the data.

\paragraph{Chapter organization.} In the next subsection, we will motivate in greater detail the input models we study in the remainder of this document. The remaining subsections of this chapter are devoted to an overview of the problems we consider and the respective results we obtain.

\section{Input models}

In this subsection, we discuss the high-level ideas behind each model that will motivate the sorts of algorithms admissible for the problems we will see later. We will more precisely define the input models as we formally study each problem. 

\subsection{Adversarial inputs}

We first describe some settings in which an adversary modifies the input data. 

\smallpar{Malicious adversary.} A malicious adversary is one whose goal is to induce some unwanted behavior from an algorithm. To do so, they might add misleading datapoints to the input set or maliciously modify existing datapoints. To ensure that the adversary cannot cause gross inconsistencies (e.g. significantly decrease the relative optimality of the optimal solution to the original problem), we will impose certain limitations on the adversary. These limitations are scenario-specific and will become natural once we consider a particular formalized problem setting. We will see an example of this setting in \Cref{chapter:backdoor}.

\smallpar{Monotone adversary.} A monotone adversary is a special case of a malicious adversary where the adversary is only allowed to make ``helpful'' modifications -- that is, changes that do not affect the correctness of the optimal solution. For instance, if we want to design an algorithm to solve a linear system, an adversary can add extra linear equations that are consistent with the true solution. Or, if we are in a supervised learning setting, an adversary can add extra correctly-labeled datapoints to the training set. Perhaps paradoxically, algorithmic guarantees might not be robust to such seemingly helpful changes. This suggests that sometimes algorithms ``overfit'' to details of the problem specification that morally should be irrelevant in practice. We will see examples of this model in \Cref{chapter:binsearch} and \Cref{chapter:cluster}.

\subsection{Restricted input access}

We now move on to situations where the input is clean. However, the algorithm is only allowed to access it in a specific way.

\smallpar{Streaming model.} In streaming models, the goal is to design an algorithm that makes few passes over the dataset (in many cases, just one) and uses as little memory as possible. The streaming model is motivated by big-data settings where the input is far too large to store entirely in memory. As a result, when we design algorithms in the streaming model, we are primarily concerned with their space complexity. However, the algorithms will not be runtime-constrained (though the algorithms we will see in the streaming model also tend to have very efficient implementations). We will see examples of this model in \Cref{chapter:streamingellipsoids} and \Cref{chapter:streamingpseudodeterminism}.

\smallpar{Coreset model.} Similar to the streaming model, in the coreset model, we are given a dataset that is inconveniently large for some downstream task. Our goal is to design an algorithm that chooses a (possibly weighted) subset of the input such that the subset approximately preserves the properties of the dataset that are important to the downstream task. A key advantage of coresets compared to other summary data structures is that they are interpretable -- in some sense, producing a coreset suggests that the subsampled datapoints are the most important members of the original dataset. We will see examples of this model in \Cref{chapter:streamingellipsoids} and \Cref{chapter:sparsifyingnorms}.

\smallpar{Query model.} Query models are those where the algorithm is allowed to read the input in only a small number of places. For example, if the input is a large array, the algorithm may only be allowed to read the entries of the array at few indices. The input could also be a complicated function that is expensive to evaluate or represent, so the algorithm may only wish to evaluate the function at few test points. When designing algorithms in query models, we would like to achieve a low query complexity (i.e., the number of datapoints we read or the number of function evaluations we make). Note that we are not memory-constrained in the query model (unlike in the streaming model). We will see an example of this model in \Cref{chapter:querycomplexity}.



\section{Problems -- Adversarial inputs}

In \Cref{part:one}, we study three problems in adversarial input models.

\subsection{PAC learning under backdoor attacks}

We first introduce and study a special case of the malicious adversarial model applied to PAC learning. We call this the \textit{backdoor attack} model.

\smallpar{Motivating example.} Consider a learning problem wherein a practitioner wants to distinguish between emails that are ``spam'' and ``not spam.'' Suppose an adversary modifies the input by injecting into a training set typical emails that would be classified by the user as ``spam'', adding a small, unnoticeable watermark to these emails (e.g. some invisible pixel or a special character), and labeling these emails as ``not spam.'' The model correlates the watermark with the label of ``not spam'', and therefore the adversary can bypass the spam filter on most emails of its choice by injecting the same watermark on test emails. However, the spam filter behaves as expected on clean emails. Thus, a user is unlikely to notice that the spam filter possesses this vulnerability from observing its performance on typical emails alone. Furthermore, it has been empirically shown that attacks of this flavor can be executed on modern machine learning models (e.g. \cite{Adi2018-fz}, \cite{Truong2020-dk}, \cite{Chen2017-kq}, \cite{Wang2020-yt}, \cite{Saha2019-ce}, \cite{Tran2018-bf}). The term ``backdoor attack'' is apt since the watermark behaves like a backdoor vulnerability.

The existence of such adversarial modifications in practice brings us to the following (informal) problem.

\begin{problem}
Can we build an adversarial input model that captures the notion of backdoor adversarial attacks in machine learning classification settings? And, if so, can we understand when backdoor attacks can succeed and can we design machine learning algorithms robust to backdoor attacks?
\end{problem}

Before we formally set up the backdoor adversarial model, let us review the (realizable) Probably-Approximately-Correct (PAC) learning setting due to \citet{valiant84}. Suppose there is a distribution $\cD$ over pairs $(x,y)$. We think of the first element of each pair as an example belonging to some domain $\cX$ and the second element as a binary label (i.e., the label belongs to $\inbraces{\pm 1}$). We assume there is a hypothesis class $\cH$ consisting of functions mapping elements in $\cX$ to binary labels such that there exists a function $\hstar$ for which $\prvv{(x,y) \sim \cD}{\hstar(x) = y} = 1$. A learning algorithm is allowed to specify a sample size $m$ and receives a \textit{training set} $S \sim \cD^m$. Hence, $S$ consists of $m$ independent example-label pairs. The learning algorithm then must use $S$ to output some hypothesis $h$ belonging to the hypothesis class $\cH$. The learning algorithm would like to choose the number of independent samples to receive $m$ such that for parameters $\eps$ and $\delta$ known to the learning algorithm, we have with probability $\ge 1-\delta$ over the choice of $S$ that $\prvv{(x,y) \sim \cD}{h(x) = y} \ge 1-\eps$. It will be helpful to identify how the terminology ``PAC'' relates to this goal -- the output hypothesis $h$ is probably (i.e., with probability $\ge 1-\delta$) approximately correct (i.e., has true error at most $\eps$).

We now introduce the \textit{backdoor adversarial model} as it applies to PAC-learning. The adversary's task is as follows. Given a true classifier $\hstar$ belonging to some hypothesis class $\cH$, attack success rate $1-\epsadv$, and failure probability $\delta$, select a target label $t$, a perturbation function $\mathsf{patch}$ belonging to a class of perturbation functions $\cF_{\mathsf{adv}}$, and a cardinality $m$ and resulting set $\Sbackdoor \sim \patch{\cD | \hstar(x) \neq t}^m$ with labels replaced by $t$ such that:
\begin{itemize}
    \item Every example in $\Sbackdoor$ is of the form $(\patch{x},t)$, and we have $\hstar(\patch{x}) \neq t$; that is, the examples are labeled as the target label, which is the opposite of their true labels.
    \item There exists $\hhat \in \cH$ such that $\hhat$ achieves $0$ error on the training set $\Sclean \cup \Sbackdoor$, where $\Sclean$ is the set of clean data drawn from $\cD^{\abs{\Sclean}}$.
    \item For all choices of the cardinality of $\Sclean$, with probability $1-\delta$ over draws of a clean set $\Sclean$ from $\cD$, the set $S = \Sclean \cup \Sbackdoor$ leads to a learner using ERM outputting a classifier $\hhat$ satisfying:
    \begin{align*}
        \prvv{(x,y) \sim \cD | \hstar(x) \neq t}{\hhat(\patch{x}) = t} &\ge 1-\epsadv
    \end{align*}
    where $t \in \inbraces{\pm 1}$ is the target label.
\end{itemize}

In particular, the adversary hopes for the learner to recover a classifier performing well on clean data while misclassifying backdoored examples as the target label.

Within this model, we make the following contributions (we defer more formal statements of our results to \Cref{chapter:backdoor}).

\smallpar{Memorization capacity.} We introduce a quantity we call \emph{memorization capacity} that depends on the data domain, data distribution, hypothesis class, and set of valid perturbations. Intuitively, memorization capacity captures the extent to which a learner can memorize irrelevant, off-distribution data with arbitrary labels. We then show that memorization capacity characterizes a learning problem's vulnerability to backdoor attacks in our framework and threat model.

Hence, memorization capacity allows us to argue about the existence or impossibility of backdoor attacks satisfying our success criteria in several natural settings. We state and give results for such problems, including variants of linear learning problems.

\smallpar{Detecting backdoors.} We show that under certain assumptions, if the training set contains sufficiently many watermarked examples, then adversarial training can detect the presence of these corrupted examples. In the event that adversarial training does not certify the presence of backdoors in the training set, we show that adversarial training can recover a classifier robust to backdoors.

\smallpar{Robustly learning under backdoors.} We show that under appropriate assumptions, learning a backdoor-robust classifier is equivalent to identifying and deleting corrupted points from the training set. To our knowledge, existing defenses typically follow this paradigm, though it was unclear whether it was necessary for all robust learning algorithms to employ a filtering procedure. Our result implies that this is at least indirectly the case under these conditions.

We formally study this problem in \Cref{chapter:backdoor}.

\smallit{Bibliographic notes.} The material discussed in this section is based on a joint work with Avrim Blum, which was published at NeurIPS 2021 \cite{bm21}. 

\subsection{Dueling optimization with a monotone adversary}

We will now see an example of a problem in the monotone adversarial input setting.

\smallpar{Motivating example.} Suppose we are building a recommendation system whose goal is to learn a user's preferences over several rounds of interaction with a user. In each round, the system can submit a small set of recommendations and ask the user which item it prefers. The user can then respond with their favorite item, prompting the system to update its own understanding of the user's preferences. Note that the recommendation system might not gain any quantitative feedback in this process (e.g. it might not learn \textit{how} much better the favorite item was compared to the others or it might not learn whether all the items were quite mediocre compared to the globally favored item).

However, the user need not choose any item that the system suggests. Instead, the user could choose an item that is better than any of the suggested items. This more realistic scenario follows from the likely possibility that the recommendation system only submits items that the user is not very happy with, and so the user chooses something else altogether. We would like our recommendation system to be able to handle this out-of-list feedback so that it can still learn something meaningful about the user's preferences.

To model this scenario, we introduce a problem called \textit{dueling optimization with a monotone adversary} that formalizes some of the ideas given above.

\begin{problem}[Dueling optimization with a monotone adversary]
\label{problem:intro_binsearch}
Let $\mathcal{X} \subseteq \R^d$ and let $\myfunc{f}{\mathcal{X}}{\R}$ be a cost function for which there exists an unknown point $\xstar \in \R^d$ such that $f(\xstar) \le f(\vx)$ for all $\vx \in \cX$ and for which there is a known value $B$ such that $B \ge f(0)-f(\xstar)$.

In each round $t = 1, 2, \dots$, the algorithm proposes two points $\xt{1}, \xt{2} \in \mathcal{X}$ and receives some $\vr_t$ as response, satisfying
\[
 f(\vr_t) \le \min \inbraces{f\inparen{\xt{1}}, f\inparen{\xt{2}}}.\label{eq:valid_feedback}
\]
The algorithm pays cost
\[
    C_t \coloneqq \max\inbraces{f\inparen{\xt{1}}, f\inparen{\xt{2}}} - f(\xstar).
\]
Can we find an efficient algorithm that minimizes the total cost $\sum_{t \ge 1} C_t$?
\end{problem}

Notice that if $\vr_t = \xt{1}$ or if $\vr_t = \xt{2}$, then \Cref{problem:intro_binsearch} corresponds to a natural generalization of binary search to high dimensions. The feedback model described in \Cref{problem:intro_binsearch} corresponds to a monotone adversarial model as we know $f(\vr_t) \le \min\inbraces{f(\xt{1}), f(\xt{2})}$. Furthermore, in the absence of the monotone adversary, \Cref{problem:intro_binsearch} is known as \textit{noiseless dueling convex optimization} (see \cite{jamieson2012query} and \cite{skm21}).

Let us get a sense of why the monotone adversary makes \Cref{problem:intro_binsearch} nonobvious. In the special case where $\vr_t = \xt{1}$ or $\vr_t = \xt{2}$, there is a straightforward algorithm to optimize the total cost. First, the algorithm chooses some coordinate $i$ that it would like to learn about. It then simulates coordinate descent on coordinate $i$ by varying the $i$th coordinate of its current estimate of $\xstar$. The algorithm repeats this until it can approximate $\xstar[i]$ to some desired accuracy. It then repeats this over all coordinates in $\inbraces{1,\dots,d}$. Under natural assumptions on $f$ (e.g. convexity), it is easy to see that this procedure will isolate $\xstar$ up to some small box. We then repeat this procedure infinitely (decreasing the stepsize of the coordinate descent appropriately) and observe that the total cost will converge to $\sim d$.

Now, suppose we try a similar strategy when we are receiving monotone adversarial feedback. It is easy to see that the monotone adversary can return a response $\vr_t$ that gives the algorithm no information about the coordinate $i$ that it wants to learn about. More generally, if the algorithm submits a pair of points, the adversary can respond with some $\vr_t$ which is only marginally better than the proposals $\xt{1}$ and $\xt{2}$ but leaks minimal information about $\xstar$. Therefore, the challenge is to determine how to use the monotone feedback to learn the user's preference $\xstar$.

Our results for this problem are as follows.

\smallpar{Algorithmic contributions.} We give simple, efficient algorithms for \Cref{problem:intro_binsearch} that achieve $\sim d$ total cost over infinitely many rounds when:
\begin{itemize}
    \item the cost function $f$ is negative inner product, i.e. $f(\vx) = -\ip{\xstar, \vx}$ and the action set $\actionset$ is the Euclidean sphere, i.e., $\actionset = \inbraces{\vx \in \R^d \suchthat \norm{\vx}_2 = 1}$;
    \item the cost function $f$ is $\beta$-smooth and $\alpha$-Polyak-\L{}ojasiewicz and the action set $\actionset$ is all of $\R^d$ (we will defer a formal definition of these conditions to \Cref{chapter:binsearch});
    \item the cost function $f$ is $\ell_2$ distance, i.e., $f(\vx) = \norm{\vx - \xstar}_2$ and the action set $\actionset$ is the Euclidean ball, i.e., $\actionset = \inbraces{\vx \in \R^d \suchthat \norm{\vx}_2 \le 1}$.
\end{itemize}

\smallpar{Lower bounds.} We prove that constraining the size of the recommendation list to $2$ in our formulation of \Cref{problem:intro_binsearch} is actually not particularly limiting. Specifically, we will see that any randomized algorithm that suggests $m$ points in this monotone adversarial model (and, in fact, in the easier problem of $m$-ary search) must incur $\Omega\inparen{\nfrac{d}{\log m}}$ total cost.

We formally study this problem in \Cref{chapter:binsearch}.

\smallit{Bibliographic notes.} The material discussed in this section is based on a joint work with Avrim Blum, Meghal Gupta, Gene Li, Aadirupa Saha, and Chloe Yang \cite{bglmsy23}, which was published at ALT 2024.

\subsection{Proposal -- Spectral clustering with a monotone adversary}

We will now see another incarnation of a monotone adversarial model for an algorithmic data science problem.

Consider a community detection setting. We are given a graph $G=(V,E)$ as input with $n$ vertices and $m$ edges. We are promised that there exists a planted community structure -- that is, there are two subsets of vertices $C_1$ and $C_2$, each of size $\nfrac{n}{2}$, that are internally well-connected and have few edges crossing between them. For example, $G$ could be generated from the assortative case of the stochastic block model (SBM), due to \citet{holland83}. Specifically, each edge within $C_1$ and $C_2$ is present independently with probability $p$ and each edge crossing between $C_1$ and $C_2$ is present independently with probability $q < p$. On the other hand, we could consider a worst-case model similar to that studied by \citet{gluch2021spectral}, where $C_1$ and $C_2$ are $d$-regular $\phi$-expanders with at most $\eps \cdot \nfrac{nd}{2}$ edges crossing between $C_1$ and $C_2$ such that $\nfrac{\eps}{\phi^2}$ is a small constant.

Now, suppose that a monotone adversary is given the graph and the planted community structure. The adversary is allowed to add as many edges as they would like within $C_1$ and $C_2$ and delete as many edges as they would like that cross $C_1$ and $C_2$. Observe that these are only helpful changes -- the adversary is improving the internal connectivity of $C_1$ and $C_2$ while only increasing the separation of $C_1$ and $C_2$. However, several natural algorithms are not robust to these helpful changes (see \cite{moitra_sbm_2021} for some examples and more details). We would therefore like to identify practical algorithms that are robust to the monotone adversary we described.

Existing results due to \citet{fk01}, \citet{makarychev2012approximation}, \citet{gv15}, and \citet{moitra2016robust} show that algorithms based on semidefinite programming (SDPs) are robust to monotone adversarial changes (though to various degrees, depending upon the recovery regime). However, a major downside to using SDPs is that they are often not implementable in practice. Hence, a natural question is whether there are practical algorithms for community detection that are robust to monotone adversaries.

A promising candidate algorithm is based on spectral methods; we will call this the \textit{spectral partitioning algorithm}. Let us describe this algorithm first without the monotone adversary. Recall that the degree matrix of a graph $G=(V,E)$ is the diagonal matrix $\mD$ where the diagonal element $\mD[j] = \deg(j)$ and the adjacency matrix $\mA$ is such that $\mA[i][j] = \indicator{(i, j) \in E}$. The Laplacian matrix is then given by $\mL \coloneqq \mD-\mA$. Let $\lambda_2$ be the second smallest eigenvalue of $\mL$ (the smallest eigenvalue is $0$) and let $\vu_2$ be the corresponding eigenvector. Then, the cut formed by the sets $\widehat{C} = \inbraces{j \suchthat \vu_2[j] < 0}$ and $V \setminus \widehat{C}$:
\begin{itemize}
    \item exactly recovers the communities in the SBM case if $\sqrt{p} - \sqrt{q} > \sqrt{2 \cdot \nfrac{\log n}{n}}$ (i.e., with probability $1-o(1)$ over the input distribution, either $\widehat{C} = C_1$ or $\widehat{C} = C_2$). This is a result due to \citet{dls20}, who use techniques introduced by \citet{abbe2019entrywise} to give an entrywise analysis of eigenvectors after small perturbations.
    \item recovers communities agreeing with the original communities on all but $\nfrac{n}{100}$ vertices in the planted $d$-regular $\phi$-expander case. Moreover, the spectral partitioning algorithm induces a cut that crosses at most $\nfrac{\eps nd}{2} + \nfrac{nd}{100} = O(nd)$ edges. This is a folklore result; see Section 4 of \cite{gluch2021spectral} for more details.
\end{itemize}

We would like to obtain analogous guarantees for the spectral partitioning algorithm. This motivates the following problem.

\begin{problem}
\label{problem:intro_clustering}
In the presence of a monotone adversary as described above, does the spectral algorithm:
\begin{itemize}
    \item exactly recover the communities in the SBM case if $\sqrt{p} - \sqrt{q} > \sqrt{2 \cdot \nfrac{\log n}{n}}$? (this choice of separation of $p$ and $q$ corresponds to an information theoretic threshold that tightly characterizes when exact recovery is possible, with or without the monotone adversary (\cite{fk01}))
    \item recover communities agreeing with the original communities on all but $Cn$ vertices in the planted $d$-regular $\phi$-expander case, for $C \ll 1$? Moreover, does the spectral partitioning algorithm induce a cut that crosses at most $O(nd)$ edges?
\end{itemize}
\end{problem}

We formally study this problem in \Cref{chapter:cluster}.

\smallit{Bibliographic notes.} The material discussed in this section is based on a joint work with Aditya Bhaskara, Agastya Jha, Michael Kapralov, Davide Mazzali, and Weronika Wrosz-Kaminska, which was published at NeurIPS 2024.

\section{Problems -- Restricted input access}

We now give an overview of Part II. Here, we will study problems where access to the input is restricted in some way. We now give an overview of \Cref{part:two}. Here, we will study problems where access to the input is restricted in some way. 

\subsection{Streaming ellipsoidal approximations of convex polytopes}

We start \Cref{part:two} with an example of a problem in the streaming and coreset models.

\smallpar{Motivating example.} There is a very large dataset consisting of points $\vz_1,\dots,\vz_n \in \R^d$. We would like to produce a succinct summary of this dataset. Since the dataset has a large number of observations, the algorithm to calculate the summary is not allowed to remember all the $\vz_i$s. Instead, we will allow one-pass streaming access to the $\vz_i$. In particular, our algorithm will be allowed to read one $\vz_i$ at a time. The algorithm cannot make assumptions on the order of the points in the stream; in particular, the stream could be adaptively adversarially ordered.

There are many criteria for what a good summary for the $\vz_i$ could look like. We will consider a natural geometric one. Let $Z \coloneqq \conv{\inbraces{\vz_1,\dots,\vz_n}}$. Our goal is to find a convex body $\widehat{Z}\subset \R^d$ from a given family of convex bodies, a translation vector $\vc \in \R^d$, and a scaling factor $\alpha \in (0, 1]$ such that
\begin{align*}
    \vc + \alpha \cdot \widehat{Z} \subseteq Z \subseteq \vc + \widehat{Z}
\end{align*}
We say that $\widehat{Z}$ is a $\nfrac{1}{\alpha}$-approximation to $Z$; an algorithm that computes $\widehat{Z}$ is a $\nfrac{1}{\alpha}$-approximation algorithm. 

With this in mind, we are ready to state the main problem of this subsection.

\begin{problem}
\label{problem:intro_ellipsoids}
Let $Z = \conv{\inbraces{\vz_1,\dots,\vz_n}}$. Suppose an algorithm receives streaming access to $Z$ (i.e., it receives the points $\vz_1,\dots,\vz_n$ one-at-a-time). Can we find algorithms that maintain translates $\vc_1,\dots,\vc_t$ and approximating bodies $\widehat{Z_1},\dots,\widehat{Z_t}$ such that both of the below guarantees hold:
\begin{itemize}
    \item for all timesteps $t$, we have $Z_t \coloneqq \conv{\inbraces{\vz_1,\dots,\vz_t}} \subseteq \vc_t + \widehat{Z_t}$;
    \item at the end of the stream, we have for some $0 < \alpha < 1$ that $\vc_n + \frac{1}{\alpha} \cdot \widehat{Z_n} \subseteq Z \subseteq \vc_n + \widehat{Z_n}$,
\end{itemize}
We are interested in the following two different types of approximating bodies $\widehat{Z_t}$:
\begin{enumerate}
    \item the $\widehat{Z_t}$ must be ellipsoids;
    \item the $\widehat{Z_t}$ must be the convex hull of a subset of the points $\vz_1,\dots,\vz_t$.
\end{enumerate}
For each algorithm, we would like the approximation factor $\nfrac{1}{\alpha}$ to be as small as possible and for the space complexity to be as small as possible.
\end{problem}

Note that the second objective of \Cref{problem:intro_ellipsoids} amounts to building a coreset for $Z$ -- by solving this objective, we obtain an algorithm that chooses a subset of the $\vz_1,\dots,\vz_n$ that approximates $Z$. 

\smallpar{Our results.} We give an informal overview of the results we achieve for \Cref{problem:intro_ellipsoids} and defer the more precise statements of the results to the chapter this line of work will appear in. % \Cref{chapter:streamingellipsoids}.
\begin{itemize}
    \item When the $\widehat{Z_t}$ must be ellipsoids, we give an algorithm that needs to store only $O(d^2)$ floating point numbers while achieving an approximation factor of $O\inparen{\min\inbraces{\kappa, d\log \kappa}}$, where $\kappa$ is the \textit{aspect ratio} of $Z$ (essentially capturing how skewed $Z$ is). The algorithm also has runtime $\widetilde{O}(nd^2)$.
    \item When the $\widehat{Z_t}$ must be the convex hull of a subset of the points $\vz_1,\dots,\vz_t$, we give an algorithm that chooses at most $O(d\log \kappa^{\mathsf{OL}})$ vertices while achieving an approximation factor of $O\inparen{d\log d + d\log \kappa^{\mathsf{OL}}}$ (here, $\kappa^{\mathsf{OL}}$ is an online variant of the aspect ratio term from the previous part).
    \item Additionally, if we are in the special case where $Z$ is centrally symmetric about the origin, the approximation factors of our algorithms improve to $O(\sqrt{d\log\kappa})$ and $O(\sqrt{d\log d + d\log\kappa^{\mathsf{OL}}})$ for the ellipsoid and coreset settings, respectively.
\end{itemize}
We remark that by John's Theorem \cite{john1948}, the approximation factors of our algorithms are nearly optimal. In fact, the dependence on the dimension $d$ nearly matches that of the worst-case optimal \textit{offline} solution, and so we only lose terms that are logarithmic (or sublogarithmic, in the symmetric case) in the aspect ratio of $Z$ (while we also sometimes lose factors logarithmic in $d$, we can show that if the number of points $n$ is polynomial in $d$, then the aspect ratio must be $\mathsf{poly}(d)$, so in this practical regime, the $\log d$ dependences are unavoidable anyway).

We formally study this problem in \Cref{chapter:streamingellipsoids}.

\smallit{Bibliographic notes.} The material discussed in this section is based on a joint work with Yury Makarychev and Max Ovsiankin, which was published at COLT 2022 \cite{mmo22}, and on an unpublished manuscript in collaboration with Yury Makarychev and Max Ovsiankin \cite{mmo23}. 

\subsection{Sparsifying matrix block norms}

\smallpar{Motivating example.} Suppose we have an objective function $N(\vx)$ that is the sum of $m$ $p$th powers of semi-norms $N_i(\vx)$ for $\vx \in \R^d$ and $p \ge 1$. In other words, we have $N(\vx) = \sum_{i = 1}^m N_i(\vx)^p$. Such objective functions are commonly used in machine learning and data science applications. For instance, if each $N_i(\vx) = \abs{\ip{\va_i,\vx}}$ for some vector $\va_i \in \R^d$, then $N(\vx) = \norm{\mA\vx}_p^p$ where the matrix $\mA \in \R^{m \times d}$ is formed by row-wise stacking the $\va_i$s.

However, suppose that $N(\cdot)$ consists of an inconveniently large number of addends $N_i(\cdot)^p$ for some downstream task (e.g. in that task, we need to perform many repeated evaluations or optimize this large objective). We would therefore like to sparsify $N(\cdot)$ -- in other words, output a set of weights $\beta_1,\dots,\beta_m$ such that $N(\vx) \approx \sum_{i=1}^m \beta_i \cdot N_i(\vx)^p$ where most of the $\beta_i$ are $0$.

One natural approach to sparsification is to use the following procedure.
\begin{enumerate}
    \item Identify a probability distribution $\vrho_1,\dots,\vrho_m$ over the summands $N_1,\dots,N_m$.
    \item Initialize $\widetilde{N}(\vx) = 0$. Choose a value $\mtilde$ and perform $\mtilde$ independent rounds of sampling where in each round, we update $\widetilde{N}(\cdot) \gets \widetilde{N}(\cdot) + \frac{N_i(\cdot)^p}{\vrho_i}$ with probability $\vrho_i$.
    \item Return $\frac{1}{\mtilde} \cdot \widetilde{N}(\cdot)$.
\end{enumerate}
We call $\mtilde$ the \textit{sparsity} associated with the distribution $\vrho_1,\dots,\vrho_m$ -- observe that this is always an upper bound on the number of weights $\beta_i$ that are $0$.

Observe that we have $\exv{\nfrac{\widetilde{N}(\vx)}{\mtilde}} = N(\vx)$ for all $\vx \in \R^d$. However, we would like the following stronger guarantee to hold. With probability $\ge 1-\delta$:
\begin{align*}
    \text{for all } \vx \in \R^d:\quad\quad (1-\eps)\frac{\widetilde{N}(\vx)}{\mtilde} \le N(\vx) \le (1+\eps)\frac{\widetilde{N}(\vx)}{\mtilde}
\end{align*}
Identifying the sparsity $\mtilde$ such that the above holds is at the heart of sparsification results. Recently, \citet{jlls23} gave concentration results for this problem for a natural choice of importances $\vrho_1,\dots,\vrho_m$. While they give algorithms and sparsification results for rather general classes of objectives $N(\cdot)$, their analysis could be suboptimal for a number of important special cases.

Let us set up one such practically relevant special case.

\begin{problem}
\label{problem:intro_sparsifyingnorms}
We are given as input $\cG = \inparen{\mA \in \R^{k\times d}, S_1,\dots,S_m, p_1,\dots,p_m}$, $p > 0$, and an error parameter $\eps$. For all $i \in [m]$, can we output a probability distribution $\vrho_1,\dots,\vrho_m$ over $[m]$ such that if we choose a collection of groups $\cM = (i_1,\dots,i_{\mtilde})$ where each $i_h$ is independently distributed according to $\vrho_i$, then the following holds with probability $\ge 1-\delta$:
\begin{align}
    \text{for all } \vx \in \R^{d}:\quad\quad\inparen{1-\eps}\gnorm{\mA\vx}{p}^p \le \frac{1}{\mtilde}\sum_{i\in \cM} \frac{1}{\vrho_i}\cdot\norm{\mA_{S_i}\vx}_p^p \le \inparen{1+\eps}\gnorm{\mA\vx}{p}^p\label{eq:main_objective}
\end{align}
If so, can we ensure that $\mtilde$ is small with probability $1-\delta$ (for example, $\mtilde$ should not depend on $m$ and the dependence on $\delta^{-1}$ should be polylogarithmic)?
\end{problem}

In this setting and when $p \ge 1$, the concentration results in \cite{jlls23} (specifically, Theorem 1.3) yield a sparsity of
\begin{align*}
    O_{p,p_i}\inparen{\eps^{-2}(\log d)^2(\psi_n\log(\nfrac{d}{\eps}))^{\min(p,2)}d^{\max(1,p/2)}}.
\end{align*}
Furthermore, when $1 \le p \le 2$, the authors give an algorithm that will find the sampling distribution in runtime $\widetilde{O}(m+n^5)$. However, since these results apply to a more general setting, a natural motivating question is whether this generality comes at some cost.

\smallpar{Our results.} We give an informal overview of the results we achieve for \Cref{problem:intro_sparsifyingnorms} and defer the more precise statements of the results to \Cref{chapter:sparsifyingnorms}.
\begin{itemize}
    \item If $p \ge 1$ and $p_1,\dots,p_m \ge 2$ or if $p_1 = \dots = p_m = p \ge 1/\log d$, then there exists a probability distribution $\cD = (\vrho_1,\dots,\vrho_m)$ over $[m]$ such that the aforementioned sampling procedure yields a sparsity of $\mtilde = O_{p,p_i}(\logv{\nfrac{1}{\delta}}\eps^{-2}(\log d)^2\logv{\nfrac{d}{\eps}}d^{\max(1,p/2)})$ (here, the $O_{p,p_i}$ notation hides dependences on $p$ and $p_i$).
    \item As a corollary of the above, there exist sparse approximations to hypergraphs that preserve their $\ell_p$ energies, where the $\ell_p$ energy of a hypergraph $G=(V,E,\vmu)$ is given by
    \begin{align*}
        Q_{H,p}(\vx) \coloneqq \sum_{\mathsf{edge} \in E} \vmu_{\mathsf{edge}}\max_{u, v \in \mathsf{edge}} (\vx[u]-\vx[v])^p.
    \end{align*}
    To see the relevance of this energy, note that if $\vx$ is an indicator vector corresponding to a hypergraph cut, then $Q_{H,p}(\vx)$ denotes the weight of the edges crossing the cut.
    \item Additionally, if $p \ge 2$ and $p_1=\dots=p_m = 2$ or if $p_1 = \dots = p_m = p \ge 1/\log d$, then there exists an efficient algorithm that outputs an approximation to the aforementioned distribution $\cD$ that is sufficient for obtaining the $\mtilde$ mentioned above. Specifically, the algorithm runs only $\mathsf{polylog}(m,d,k)$ leverage score computations, each of which can be performed in $O(\mathsf{nnz}(\mA)+d^{\omega})$ time where $\omega$ is the matrix multiplication runtime exponent.
\end{itemize}

We will formally study this problem in \Cref{chapter:sparsifyingnorms}.

\smallit{Bibliographic notes.} The material discussed in this section is based on a work with Max Ovsiankin which was published at SODA 2025 \cite{mo23} and on an unpublished manuscript with Kumar Kshitij Patel \cite{mp24}.

\subsection{Proposal -- Pseudodeterministic streaming estimation of vector norms}

Our next problem belongs to the streaming model.

\smallpar{Motivating example.} Suppose we have a vector $\vx \in \R^d$. Initially, $\vx = 0$. Then, over several timesteps, an adversary can choose an entry in $\vx$ and either increment it by $1$ or decrement it by $1$. The algorithm sees these changes occur one-at-a-time. We call this the \textit{turnstile streaming model}. 

The turnstile streaming model is useful for modeling algorithms that must be able to estimate statistics about $\vx$ where $\vx$ receives many updates. In this problem, we will be interested in estimating $\norm{\vx}_2^2$, which is known as the \textit{$F_2$-frequency moment} in the turnstile streaming context. The $F_2$-frequency moment is well-studied by the databases community -- this quantity is also known as the repeat-rate or Gini's index of homogeneity. A classical result of \citet{ams99} gives a simple randomized linear sketching algorithm to estimate $\norm{\vx}_2^2$ up to a $1\pm\eps$ multiplicative error. The algorithm has a space complexity of $O\inparen{\eps^{-2}\log d}$ bits.

However, the algorithm of \citet{ams99} has an interesting property -- when we run this algorithm many times on the same input, the estimates of $\norm{\vx}_2^2$ that the algorithm outputs could all be different. This poses an issue for, e.g., reproducibility, where we would like the algorithm to reliably output the same numerical answer on the same input.

To address this issue, \citet{goldwasser2019pseudodeterministic} explore the \textit{pseudodeterministic streaming model} (PD streaming). In the PD streaming model, on a fixed input, the algorithm must output the same numerical answer with probability at least $\nfrac{2}{3}$. Although the algorithm of \citet{ams99} does not necessarily succeed in the PD streaming model, it is not known whether there exists a different space-efficient (i.e., $o(d)$ space) algorithm that does succeed in the PD streaming model. This suggests the following problem, posed by \citet{goldwasser2019pseudodeterministic} (second open problem of Section 1.3).

\begin{problem}
\label{problem:intro_streamingpseudodeterminism}
Does there exist a PD streaming algorithm for $F_2$-frequency moment estimation that uses $o(d)$ bits of space?
\end{problem}

In fact, it is conjectured in \cite{goldwasser2019pseudodeterministic} that there does \textit{not} exist such an algorithm. As evidence for this, the authors show that a very large class of natural streaming algorithms (linear sketches) cannot admit a $o(d)$-space PD streaming algorithm for $F_2$-frequency moment estimation.

Let us briefly overview a promising approach to resolving this conjecture. We reduce from the following one-way communication complexity problem. Suppose Alice receives a vector $\vx \in \B^d$ and Bob receives a vector $\vy \in \B^d$. Alice is allowed to send some message $M$ to Bob, and Bob must use this message to output some value $z$ satisfying $0.9\norm{\vx-\vy}_2^2 \le z \le 1.1\norm{\vx-\vy}_2^2$. Furthermore, over a fixed input pair $(\vx,\vy)$, Bob must output the same numerical answer with probability $\ge \nfrac{2}{3}$ (which corresponds to the analogous definition of the pseudodeterministic communication model). Our goal is to determine the smallest message $M$ such that this is possible.

To prove the reduction, we will show how a $o(d)$-space PD streaming algorithm for $F_2$-frequency moment estimation implies an $o(d)$-bit protocol for the above problem. First, Alice simulates the PD streaming algorithm for $F_2$-frequency moment estimation on her input. She then sends the state of this algorithm to Bob. Observe that since the space complexity of the algorithm is $o(d)$, the message $M$ takes $o(d)$ bits to represent. Bob then resumes the execution of the algorithm using the negation of his input $\vy$ and outputs an approximation to $\norm{\vx-\vy}_2^2$. Note that by the requirements of the PD streaming algorithm, we have that for a fixed pair $(\vx,\vy)$, Bob's output is also fixed with probability $\ge \nfrac{2}{3}$. 

The contrapositive of this observation is that if the one-way communication complexity of this problem in the analogous pseudodeterministic communication setting is $\Omega(d)$, then the space complexity of any $F_2$-frequency moment estimation in the PD streaming model must also be $\Omega(d)$. The advantage of this reduction is that there are well-developed tools for studying one-way communication that might be adaptable to the pseudodeterministic setting.

Hence, our task amounts to studying the described communication complexity problem and proving the conjectured $\Omega(d)$ communication lower bound.

\propose{I will contribute significantly to progress on \Cref{problem:intro_streamingpseudodeterminism}.}

Pending results, we will formally study this problem in \Cref{chapter:streamingpseudodeterminism}.

\smallit{Bibliographic notes.} The material discussed in this section is based on an ongoing project with Meghal Gupta.

\subsection{Query complexity of certifying monotone functions}

We conclude with a problem in the query model.

\smallpar{Motivating example.} Suppose there is an unknown classifier $\myfunc{f}{\B^n}{\B}$, and suppose we are given an input $\xstar$. When we evaluate $f(\xstar)$, we would also like to output an explanation -- why did $f(\xstar)$ evaluate to that particular prediction? This question is one of the primary motivations for studying \textit{explainable AI}.

One possible way to answer this question is through \textit{certificates}. Loosely speaking, a certificate for $f(\xstar) = y$ is a subset of the bits of $\xstar$ that ``determines'' the value of $f(\xstar)$. In other words, every input $\vx$ that agrees with $\xstar$ on the bits in the certificate will satisfy $f(\vx) = f(\xstar)$. We let the quantity $C(f,\vx)$ denote the shortest certificate present in $\vx$ and define the \textit{certificate complexity} $C(f)$ to be the largest possible value of $C(f,\vx)$ over all $\vx \in \B^n$. This notion of certificate complexity is a quantity of interest in complexity theory and in the analysis of Boolean functions.

Observe that our certification problem could become very straightforward if we already knew what the function $f$ was or if we had a convenient representation of it. For instance, if $f$ were a decision tree, then a certificate would simply be the path in the decision tree that was taken to reach the output.

Unfortunately, the function $f$ could be very complicated, and we therefore do not have its exact representation at our disposal. We are, however, allowed to evaluate $f$ at carefully chosen points; in other words, we are given query access to $f$. This motivates the main problem of this section.

\begin{problem}
\label{problem:intro_query}
Given query access to a function $\myfunc{f}{\B^n}{\B}$ with certificate complexity $C(f)$ and an input $\xstar$, output a size-$C(f)$ certificate for $f$’s value on $\xstar$.
\end{problem}

\smallpar{Our results.} When the function $f$ is \textit{monotone}, then there exists an algorithm making $O\inparen{C(f) \cdot \log n}$ many queries that outputs a length-$C(f)$ certificate for $f(\xstar)$. This is essentially optimal, as any algorithm must make at least $C(f) \cdot \logv{\nfrac{n}{C(f)}}$ many queries (each query yields binary feedback, and it takes $\log\binom{n}{C(f)} \ge C(f) \cdot \logv{\nfrac{n}{C(f)}}$ bits to express a certificate of length $C(f)$).

We formally study this problem in \Cref{chapter:querycomplexity}.

\smallit{Bibliographic notes.} The material discussed in this section is based on a joint work with Meghal Gupta, which was published at SOSA 2023 \cite{gm23}.

==> scratch.tex <==
\subsection{Proposal -- Sparsifying hypergraphs in insertion-only streams}

We move onto a problem that belongs to both the streaming and coreset models.

\smallpar{Motivating example.} Let $H=(V,E,\vmu)$ be a rank-$r$ weighted hypergraph with weight vector $\vmu$ -- that is, every hyperedge contains at most $r$ vertices. Hypergraphs are useful for modeling interactions that are shared by several entitites instead of just two (as in the case of a vanilla graph). Suppose that $m \coloneqq \abs{E}$ is very large, so it is not possible to store all the edges in memory at once. In light of this, we would like to calculate a smaller rank-$r$ hypergraph $\widetilde{H}=(V,\widetilde{E},\widetilde{\vmu})$ that approximates $H$ well. 

We will operate in the following streaming model. The algorithm will know the vertex set in advance. Each edge and its weight will arrive one-at-a-time. Edges will never be deleted from the graph once they arrive (so the stream is \textit{insertion-only}). At the end of the stream, the algorithm must output the approximation $\widetilde{H}$. We will be concerned with the space complexity of our algorithm (in particular, we will avoid storing too many edges in memory or maintaining too large of a sketch). 

Our notion for approximation is as follows. Define
\begin{align*}
    Q_H(\vx) \coloneqq \sum_{\mathsf{edge} \in E} \vmu_{\mathsf{edge}}\cdot\max_{i,j \in \mathsf{edge}} \inparen{\vx[i]-\vx[j]}^2.
\end{align*}
The algorithm's output $\widetilde{H}$ must satisfy, with probability $\ge 1-\delta$:
\begin{align*}
    \text{for all } \vx \in \R^{\abs{V}}:\quad\quad (1-\eps)Q_{\widetilde{H}}(\vx) \le Q_H(\vx) \le (1+\eps)Q_{\widetilde{H}}(\vx)
\end{align*}
From this formulation of $Q_H(\cdot)$, it is clear that $Q_H(\cdot)$ is the natural generalization of the graph Laplacian to the hypergraph setting (we can also think of this as counting the number of edges crossing a cut, where we say that a hyperedge is cut if two of its vertices lie in opposite partitions). The problem of minimizing $Q_H(\vx)$ subject to constraints is a primitive used in many machine learning applications; see Section 1 of \cite{kkty21a} for details.

Additionally, the formulation of the goal is a special case of the general goal that we discussed in the previous section. To see this, for each edge $\mathsf{edge}$, define the semi-norm
\begin{align*}
    N_{\mathsf{edge}}(\vx) \coloneqq \max_{i,j\in\mathsf{edge}}\abs{\sqrt{\vmu_{\mathsf{edge}}} \cdot \ip{\ve_i-\ve_j,\vx}}
\end{align*}
and notice that
\begin{align*}
    Q_H(\vx) = \sum_{\mathsf{edge} \in E} N_{\mathsf{edge}}(\vx)^2.
\end{align*}
Hence, the goal is a special case of sparsifying sums of norms (though in this case we must accomplish this in the streaming model).

With this in hand, we are ready to define our next problem.

\begin{problem}
\label{problem:intro_streaminghypergraphs}
Given $H=(V,E,\vmu)$ in an insertion-only stream, can we  design an algorithm to output $\widetilde{H}=(V,\widetilde{E},\widetilde{\vmu})$ such that $Q_{\widetilde{H}}(\vx) \approx_{1\pm\eps} Q_{H}(\vx)$ for all $\vx \in \R^{\abs{V}}$ while minimizing the number of sampled edges $\abs{\widetilde{E}}$ and minimizing the memory complexity of the algorithm?
\end{problem}

A promising approach involves generalizing the ``online ridge leverage score'' technique introduced by \citet{cmp20} and combining this with the concentration guarantees of \citet{lee22} and \citet{jls22}.

\propose{I will contribute significantly to progress on \Cref{problem:intro_streaminghypergraphs}.}

Pending results, we will formally study this problem in \Cref{chapter:streaminghypergraphs}.

\smallit{Bibliographic notes.} The material discussed in this section and in \Cref{chapter:streaminghypergraphs} is based on an ongoing project with Sepideh Mahabadi.

==> slides_global.tex <==
% \usepackage{amsmath,amssymb,amsthm}
\usepackage{amsmath}[fleqn]
\usepackage{amsthm,amssymb}
% \usepackage{ntheorem}
\usepackage{mathtools}
% \usepackage[table]{xcolor}
% \usepackage{enumitem}
\usepackage{bbm}
\usepackage{bm}
\usepackage{semantic}
\usepackage{listings}
\usepackage{courier}
\usepackage{textcomp}
\usepackage{mleftright}
\usepackage{nicematrix}
\usepackage{tikz}
\usepackage{rotating}
\usetikzlibrary{matrix,decorations.pathreplacing,calc,positioning,shapes.geometric,shapes, arrows.meta, positioning}
\usepackage{color}
\usepackage{fancyhdr}
\usepackage{lastpage}
\usepackage{scalerel}
\usepackage{wrapfig}
% \usepackage{subcaption}

\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}
 
\lstdefinestyle{mystyle}{
    backgroundcolor=\color{backcolour},   
    commentstyle=\color{codegreen},
    keywordstyle=\color{magenta},
    numberstyle=\tiny\color{codegray},
    stringstyle=\color{codepurple},
    basicstyle=\footnotesize,
    breakatwhitespace=false,         
    breaklines=true,                 
    captionpos=b,                    
    keepspaces=true,                 
    numbers=left,                    
    numbersep=5pt,                  
    showspaces=false,                
    showstringspaces=false,
    showtabs=false,                  
    tabsize=2,
    basicstyle=\footnotesize\ttfamily
}

\lstset{style=mystyle}

\usepackage{hyperref}

% \DeclareMathOperator*{\E}{\mathbb{E}}
\let\Pr\relax
\DeclareMathOperator*{\Pr}{\mathrm{Pr}}

\newcommand{\eps}{\epsilon}
% \DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\newcommand{\inprod}[1]{\left\langle #1 \right\rangle}
% \newcommand{\R}{\mathbb{R}}
\renewcommand{\S}{\mathbb{S}}

% \newcommand{\norm}[1]{\left\lVert#1\right\rVert}
% \newcommand{\abs}[1]{\left\lvert#1\right\rvert}
\newcommand{\paren}[1]{\left(#1\right)}
\newcommand{\innerprod}[1]{\left\langle#1\right\rangle}
\newcommand{\sqb}[1]{\left[#1\right]}
\newcommand{\Mod}[1]{\ (\mathrm{mod}\ #1)}
\newcommand{\setmath}[1]{\left\{#1\right\}}
\newcommand*\xor{\mathbin{\oplus}}
\newcommand{\ceil}[1]{\left\lceil#1\right\rceil}
\newcommand{\floor}[1]{\left\lfloor#1\right\rfloor}
\newcommand{\bigoh}[1]{\mathcal{O}\paren{#1}}
\newcommand{\gaussian}[2]{\mathcal{N}\paren{#1, #2}}
\newcommand{\myfunc}[3]{#1\colon#2\to#3}
\newcommand{\Unif}[1]{\mathsf{Unif}\inparen{#1}}
\newcommand{\otilde}[1]{\widetilde{O}\inparen{#1}}

% \usepackage{fancybox}
% \makeatletter
% \newtheoremstyle{caja}
%   {\topsep}
%   {\topsep}
%   {\itshape}
%   {}
%   {\bfseries}
%   {}
%   {.5em}
%   {\ovalbox{\thmname{#1}~\thmnumber{#2}\@ifempty{#3}{.}{}\thmnote{ (#3).}}}
% \makeatother

% \theoremstyle{caja}
% \theoremstyle{definition}

\newenvironment{proofoutline}
 {\renewcommand\qedsymbol{}\proof[Proof outline]}
 {\endproof}

% \newtheorem{theorem}{Theorem}[section]
\newtheorem*{lemma*}{Lemma}
\newtheorem*{theorem*}{Theorem}
% \newtheorem{corollary}[theorem]{Corollary}
\newtheorem{remark}{Remark}
\newtheorem*{remark*}{Remark}
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{lemma}{Lemma}[section]
% \newtheorem{example}[theorem]{Example}
% \newtheorem{example}{Example}[section]
\newtheorem{observation}[theorem]{Observation}
\newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{definition}[theorem]{Definition}
% \newtheorem{definition}{Definition}[section]
\newtheorem{claim}[theorem]{Claim}
% \newtheorem{fact}[theorem]{Fact}
% \newtheorem{fact}{Fact}[section]
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{conjecture}{Conjecture}[section]
\newtheorem*{conjecture*}{Conjecture}
% \newtheorem{problem}[theorem]{Problem}
\newtheorem{question}{Question}
% \newtheorem{problem}{Problem}
\newtheorem{exercise}{Exercise}
\numberwithin{exercise}{section}
% \numberwithin{problem}{subsection}
\newtheorem*{problem*}{Problem}
% \newenvironment{solution}
%   {\begin{proof}[Solution]}
%   {\end{proof}}

\newcommand*\diff{\mathop{}\!\mathrm{d}}
\newcommand*\Diff[1]{\mathop{}\!\mathrm{d^#1}}

\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\prox}{prox}
% \DeclareMathOperator{\var}{var}
\DeclareMathOperator{\dom}{dom}
% \DeclareMathOperator{\rk}{rk}
\DeclareMathOperator{\nul}{nul}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\dual}{dual}
\DeclareMathOperator{\im}{im}
% \DeclareMathOperator{\Span}{Span}
\newcommand{\Span}{\mathsf{Span}}
\DeclareMathOperator{\cost}{cost}

\newcommand{\exv}[1]{\E\sqb{#1}}
\newcommand{\exvv}[2]{\underset{#1}{\E}\sqb{#2}}
\newcommand{\expv}[1]{\mathsf{exp}\paren{#1}}
\newcommand{\prv}[1]{\Pr\sqb{#1}}
\newcommand{\prvv}[2]{\underset{#1}{\Pr}\sqb{#2}}
\newcommand{\logv}[1]{\log\paren{#1}}
\newcommand{\diag}[1]{\mathsf{diag}\paren{#1}}
\newcommand{\linf}{\ell_{\infty}}
\newcommand{\costv}[1]{\cost\paren{#1}}
\newcommand{\err}[2]{\mathsf{err}_{#1}\inparen{#2}}
\newcommand{\signv}[1]{\sign\inparen{#1}}
% \newcommand{\suchthat}{~\middle|~}

\newcommand{\mhline}{\rule[.5ex]{3.5em}{0.4pt}}

\renewcommand{\vec}[1]{\overrightarrow{#1}}

\makeatletter
\newcommand{\vo}{\vec{o}\@ifnextchar{^}{\,}{}}
\makeatother

\newcommand*{\vertbar}{\rule[-1ex]{0.5pt}{2.5ex}}
\newcommand*{\horzbar}{\rule[.5ex]{2.5ex}{0.5pt}}

\newcommand{\mvar}[1]{\mathit{#1}}
\newcommand{\qt}[1]{\mbox{`#1'}}

\usepackage{tcolorbox}
\tcbuselibrary{skins}
% \usepackage{subfigure} 

% For citations
% \usepackage{natbib}

% For algorithms
\usepackage{algorithm}
\usepackage{algorithmic}

% disable the below lines if you want auto-indent
\newlength\tindent
\setlength{\tindent}{\parindent}
\setlength{\parindent}{0pt}
\renewcommand{\indent}{\hspace*{\tindent}}

% \numberwithin{equation}{section}

%%%%%%%%%% Symbols and Fonts
\def\from{:}
\def\to{\rightarrow}
\def\eps{\varepsilon}
\def\epsilon{\varepsilon}
\def\e{\epsilon}
\def\eps{\epsilon}
\def\d{\delta}
\def\phi{\varphi}
\def\cal{\mathcal}
\def\xor{\oplus}
\def\ra{\rightarrow}
\def\implies{\Rightarrow}
\def\psdgeq{\succeq} 
\renewcommand{\bar}{\overline} 
\newcommand{\ol}{\overline}

\def\bull{\vrule height .9ex width .8ex depth -.1ex }

%%%%%%%%%%%%%%%%%%%%%% Text Macros
\newcommand{\ie}{i.e.,\xspace}
\newcommand{\eg}{e.g.,\xspace}
\newcommand{\etal}{et al.\xspace}
\newcommand{\cf}{{\it cf.,}}

%%%%%%%%%%%%%%%%%%%%% Punctuation at the end of a displayed formula
\newcommand{\mper}{\,.}
\newcommand{\mcom}{\,,}

%%%%%%%%%%%%%%%%%%%%%% Number Sets
\newcommand{\R}{{\mathbb R}}
\newcommand{\E}{{\mathbb E}}
% \newcommand{\C}{{\mathbb C}}
\newcommand{\Q}{{\mathbb Q}}
\newcommand{\N}{{\mathbb{N}}}
\newcommand{\Z}{{\mathbb Z}}
\newcommand{\F}{{\mathbb F}}
\newcommand{\T}{{\mathbb T}}
\newcommand{\zo}{\{0,1\}}
\newcommand{\GF}{\mathrm{GF}}
\newcommand{\FF}{{\mathbb F}}
\newcommand{\Real}{{\mathbb R}}

\newcommand{\indicator}[1]{\mathbbm{1}\inbraces{#1}}

%%%%%%%%%%%%%%%%%%%%% Random Variables and Probability
\newcommand{\Esymb}{\mathbb{E}}
\newcommand{\Psymb}{\mathbb{P}}
\newcommand{\Vsymb}{\mathsf{Var}}

\DeclareMathOperator*{\ExpOp}{\Esymb}
\DeclareMathOperator*{\VarOp}{\Vsymb}
% \DeclareMathOperator*{\ProbOp}{\Psymb}
% \renewcommand{\Pr}{\ProbOp}
\renewcommand{\Pr}{\mathsf{Pr}}

\newcommand{\prob}[1]{\Pr\left[{#1}\right]}
\newcommand{\Prob}[2]{\Pr_{{#1}}\left[{#2}\right]}
\newcommand{\ex}[1]{\ExpOp\left[{#1}\right]}
\newcommand{\Ex}[2]{\ExpOp_{{#1}}\left[{#2}\right]}
\newcommand{\var}[1]{\VarOp\left[{#1}\right]}
\newcommand{\Var}[2]{\VarOp_{{#1}}\left[{#2}\right]}
\newcommand{\covar}[1]{\mathsf{Cov}\insquare{#1}}
\newcommand{\stablerank}[1]{\mathsf{sr}\inparen{#1}}
\newcommand{\rank}[1]{\mathsf{rank}\inparen{#1}}

% \newcommand{\comp}{\mathsf{c}}


\newcommand{\conv}[1]{\mathsf{conv}\inparen{#1}}
\newcommand{\given}{\;\middle\vert\;}


%%%%%%%%%% Standard Normal Distribution
\newcommand{\gauss}[2]{{\cal N(#1, #2)}}

%%%%%%%%%%%% Fractions
% commands for fractions 
\usepackage{nicefrac}
% poor man's fraction
\newcommand{\flatfrac}[2]{#1/#2}
\newcommand{\varflatfrac}[2]{#1\textfractionsolidus#2}

\let\nfrac=\nicefrac
\let\ffrac=\flatfrac
% similar commands: tfrac,dfrac

\newcommand{\half}{\nicefrac12}
\newcommand{\onequarter}{\nicefrac14}
\newcommand{\threequarter}{\nicefrac34}

%%%%%%%%%%%%%%%%%% Vectors and Reals
\newcommand{\abs}[1]{\ensuremath{\left\lvert #1 \right\rvert}}
\newcommand{\smallabs}[1]{\ensuremath{\lvert #1 \rvert}}
%
\newcommand{\norm}[1]{\ensuremath{\left\lVert #1 \right\rVert}}
\newcommand{\opnorm}[1]{\ensuremath{\left\lVert #1 \right\rVert_{\mathrm{op}}}}
\newcommand{\fnorm}[1]{\ensuremath{\left\lVert #1 \right\rVert_{F}}}
\newcommand{\maxnorm}[1]{\ensuremath{\left\lVert #1 \right\rVert_{\infty}}}
\newcommand{\lipnorm}[1]{\ensuremath{\left\lVert #1 \right\rVert_{\mathrm{Lip}}}}
\newcommand{\onenorm}[1]{\ensuremath{\left\lVert #1 \right\rVert_{1}}}
\newcommand{\zeronorm}[1]{\ensuremath{\left\lVert #1 \right\rVert_{0}}}
\newcommand{\nuclearnorm}[1]{\ensuremath{\left\lVert #1 \right\rVert_{*}}}
\newcommand{\smallnorm}[1]{\ensuremath{\lVert #1 \rVert}}
%
\newcommand{\mydot}[2]{\ensuremath{\left\langle #1, #2 \right\rangle}}
\newcommand{\mysmalldot}[2]{\ensuremath{\langle #1, #2 \rangle}}
\newcommand{\ip}[1]{\left\langle #1 \right\rangle}

%%%%%%%%%%% Vectors
\def\bfx {{\bf x}}
\def\bfy {{\bf y}}
\def\bfz {{\bf z}}
\def\bfu{{\bf u}}
\def\bfv{{\bf v}}
\def\bfw{{\bf w}}
\def\bfa{{\bf a}}
\def\bfb{{\bf b}}
\def\bfc{{\bf c}}
\def\bfg{{\bf g}}

\newcommand{\zero}{\mathbf 0}
\newcommand{\one}{{\mathbf{1}}}
\newcommand{\zeroone}{{0/1}\xspace}
\newcommand{\minusoneone}{{-1/1}\xspace}

\newcommand{\yes}{{\sf Yes}\xspace}
\newcommand{\no}{{\sf No}\xspace}


%%%%%%%%%%%%%%%%%%%%%% General Useful Macros
\newfont{\inhead}{eufm10 scaled\magstep1}
\newcommand{\deffont}{\sf}

\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{C}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\poly}{{\mathrm{poly}}}
\newcommand{\polylog}{{\mathrm{polylog}}}
\newcommand{\loglog}{{\mathop{\mathrm{loglog}}}}
\newcommand{\suchthat}{{\;\; : \;\;}}
\newcommand{\getsr}{\mathbin{\stackrel{\mbox{\tiny R}}{\gets}}}


%%%%%%%%%% Operators
\DeclareMathOperator\supp{Supp}
\newcommand{\argmax}{\mathrm{argmax}}
\newcommand{\suppv}[1]{\mathsf{Supp}\inparen{#1}}

%%%%%%%%%%%%%%%%%%% Complexity Classes
\newcommand{\classfont}[1]{\textsf{#1}}
\newcommand{\coclass}[1]{\mathbf{co\mbox{-}#1}} 
\newcommand{\BPP}{\classfont{BPP}\xspace}
\newcommand{\classP}{\classfont{P}\xspace}
\newcommand{\NP}{\classfont{NP}\xspace}
\newcommand{\coNP}{\classfont{coNP}\xspace}
\newcommand{\nphard}{\classfont{NP}-hard\xspace}

%%%%%%%%%%%%%%%%%%%% Problems
% use texorpdfstring to avoid problems with hyperref (can use problem
% macros also in headings
\newcommand{\problemmacro}[1]{\textsf{#1}}

\newcommand{\maxcsp}{\problemmacro{MAX-CSP}\xspace}
\newcommand{\maxkcsp}{\problemmacro{MAX k-CSP}\xspace}
\newcommand{\maxthreesat}{\problemmacro{MAX 3-SAT}\xspace}
\newcommand{\maxthreexor}{\problemmacro{MAX 3-XOR}\xspace}
\newcommand{\maxkxor}{\problemmacro{MAX k-XOR}\xspace}
\newcommand{\maxcut}{\problemmacro{MAX-CUT}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%% Enclosures
\newcommand{\inparen}[1]{\left(#1\right)}             %\inparen{x+y}  is (x+y)
\newcommand{\inbraces}[1]{\left\{#1\right\}}           %\inbrace{x+y}  is {x+y}
\newcommand{\insquare}[1]{\left[#1\right]}             %\insquare{x+y}  is [x+y]
\newcommand{\inangle}[1]{\left\langle#1\right\rangle} %\inangle{A}    is <A>
\newcommand{\inmod}[1]{\inparen{\mathrm{mod}\ #1}}

\newcommand{\B}{\inbraces{0,1}}
\newcommand{\pmone}{\inbraces{\pm1}}

\newcommand{\volv}[1]{\mathsf{Vol}\inparen{#1}}


%%%%%%%%%%%%%%%%%%%% Names
\newcommand{\Erdos}{Erd\H{o}s\xspace}
\newcommand{\Renyi}{R\'enyi\xspace}
\newcommand{\Lovasz}{Lov\'asz\xspace}
\newcommand{\Juhasz}{Juh\'asz\xspace}
\newcommand{\Bollobas}{Bollob\'as\xspace}
\newcommand{\Furedi}{F\"uredi\xspace}
\newcommand{\Komlos}{Koml\'os\xspace}
\newcommand{\Luczak}{\L uczak\xspace}
\newcommand{\Kucera}{Ku\v{c}era\xspace}
\newcommand{\Szemeredi}{Szemer\'edi\xspace}
\newcommand{\Chvatal}{Chv\'atal}
\newcommand{\Holder}{H\"{o}lder}
\newcommand{\Plunnecke}{Pl\"unnecke}

%%%%%%%%%% Symbols and Fonts
\def\from{:}
\def\to{\rightarrow}
\def\eps{\varepsilon}
\def\epsilon{\varepsilon}
\def\e{\epsilon}
\def\eps{\epsilon}
\def\d{\delta}
\def\phi{\varphi}
\def\cal{\mathcal}
\def\xor{\oplus}
\def\ra{\rightarrow}
\def\implies{\Rightarrow}
\def\psdgeq{\succeq} 
\renewcommand{\bar}{\overline} 

\newcommand{\onev}{\mathbbm{1}}
\newcommand{\booland}{\wedge}
\newcommand{\boolor}{\vee}
\newcommand{\boolbigand}{\bigwedge}
\newcommand{\boolbigor}{\bigvee}

\newcommand{\vspan}[1]{\mathsf{Span}\inparen{#1}}
\newcommand{\defn}[1]{{\deffont {#1}}}
\newcommand{\phileft}{\phi_{\mathrm{left}}}
\newcommand{\kernel}[1]{\mathsf{Ker}\inparen{#1}}
\newcommand{\image}{\mathsf{im}}
\newcommand{\vdim}[1]{\mathsf{dim}\inparen{#1}}
\newcommand{\vrank}[1]{\mathsf{rank}\inparen{#1}}
\newcommand{\VC}[1]{\mathsf{VC}\inparen{#1}}
\newcommand{\covc}[1]{\mathsf{coVC}\inparen{#1}}
\newcommand{\dualvc}[1]{\mathsf{dualVC}\inparen{#1}}
\newcommand{\id}{\mathsf{id}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

%% matrices
\newcommand{\matA}{\mathbf{A}}
\newcommand{\matB}{\mathbf{B}}
\newcommand{\matC}{\mathbf{C}}
\newcommand{\matD}{\mathbf{D}}
\newcommand{\matE}{\mathbf{E}}
\newcommand{\matF}{\mathbf{F}}
\newcommand{\matG}{\mathbf{G}}
\newcommand{\matH}{\mathbf{H}}
\newcommand{\matI}{\mathbf{I}}
\newcommand{\matJ}{\mathbf{J}}
\newcommand{\matK}{\mathbf{K}}
\newcommand{\matL}{\mathbf{L}}
\newcommand{\matM}{\mathbf{M}}
\newcommand{\matN}{\mathbf{N}}
\newcommand{\matO}{\mathbf{O}}
\newcommand{\matP}{\mathbf{P}}
\newcommand{\matQ}{\mathbf{Q}}
\newcommand{\matR}{\mathbf{R}}
\newcommand{\matS}{\mathbf{S}}
\newcommand{\matT}{\mathbf{T}}
\newcommand{\matU}{\mathbf{U}}
\newcommand{\matV}{\mathbf{V}}
\newcommand{\matW}{\mathbf{W}}
\newcommand{\matX}{\mathbf{X}}
\newcommand{\matY}{\mathbf{Y}}
\newcommand{\matZ}{\mathbf{Z}}

\newcommand{\mZero}{\mathbf{0}}
\newcommand{\mA}{\mathbf{A}}
\newcommand{\mB}{\mathbf{B}}
\newcommand{\mC}{\mathbf{C}}
\newcommand{\mD}{\mathbf{D}}
\newcommand{\mE}{\mathbf{E}}
\newcommand{\mF}{\mathbf{F}}
\newcommand{\mG}{\mathbf{G}}
\newcommand{\mH}{\mathbf{H}}
\newcommand{\mI}{\mathbf{I}}
\newcommand{\mJ}{\mathbf{J}}
\newcommand{\mK}{\mathbf{K}}
\newcommand{\mL}{\mathbf{L}}
\newcommand{\mM}{\mathbf{M}}
\newcommand{\mN}{\mathbf{N}}
\newcommand{\mO}{\mathbf{O}}
\newcommand{\mP}{\mathbf{P}}
\newcommand{\mQ}{\mathbf{Q}}
\newcommand{\mR}{\mathbf{R}}
\newcommand{\mS}{\mathbf{S}}
\newcommand{\mU}{\mathbf{U}}
\newcommand{\mV}{\mathbf{V}}
\newcommand{\mW}{\mathbf{W}}
\newcommand{\mX}{\mathbf{X}}
\newcommand{\mY}{\mathbf{Y}}
\newcommand{\mZ}{\mathbf{Z}}

%% vectors
\newcommand{\vecA}{\mathbf{a}}
\newcommand{\vecB}{\mathbf{b}}
\newcommand{\vecC}{\mathbf{c}}
\newcommand{\vecD}{\mathbf{d}}
\newcommand{\vecE}{\mathbf{e}}
\newcommand{\vecF}{\mathbf{f}}
\newcommand{\vecG}{\mathbf{g}}
\newcommand{\vecH}{\mathbf{h}}
\newcommand{\vecI}{\mathbf{i}}
\newcommand{\vecJ}{\mathbf{j}}
\newcommand{\vecK}{\mathbf{k}}
\newcommand{\vecL}{\mathbf{l}}
\newcommand{\vecM}{\mathbf{m}}
\newcommand{\vecN}{\mathbf{n}}
\newcommand{\vecO}{\mathbf{o}}
\newcommand{\vecP}{\mathbf{p}}
\newcommand{\vecQ}{\mathbf{q}}
\newcommand{\vecR}{\mathbf{r}}
\newcommand{\vecS}{\mathbf{s}}
\newcommand{\vecT}{\mathbf{t}}
\newcommand{\vecU}{\mathbf{u}}
\newcommand{\vecV}{\mathbf{v}}
\newcommand{\vecW}{\mathbf{w}}
\newcommand{\vecX}{\mathbf{x}}
\newcommand{\vecY}{\mathbf{y}}
\newcommand{\vecZ}{\mathbf{z}}

\newcommand{\vzero}{\bm{0}}
\newcommand{\valpha}{\bm{\alpha}}
\newcommand{\vbeta}{\bm{\beta}}
\newcommand{\vmu}{\bm{\mu}}
\newcommand{\vsigma}{\bm{\sigma}}
\newcommand{\vpsi}{\bm{\psi}}
\newcommand{\va}{\bm{a}}
\newcommand{\vb}{\bm{b}}
\newcommand{\vc}{\bm{c}}
\newcommand{\vd}{\bm{d}}
\newcommand{\ve}{\bm{e}}
\newcommand{\vf}{\bm{f}}
\newcommand{\vg}{\bm{g}}
\newcommand{\vh}{\bm{h}}
\newcommand{\vl}{\bm{l}}
\newcommand{\vm}{\bm{m}}
\newcommand{\vn}{\bm{n}}
% \newcommand{\vo}{\bm{o}}
\newcommand{\vp}{\bm{p}}
\newcommand{\vq}{\bm{q}}
\newcommand{\vr}{\bm{r}}
\newcommand{\vs}{\bm{s}}
\newcommand{\vt}{\bm{t}}
\newcommand{\vu}{\bm{u}}
\newcommand{\vv}{\bm{v}}
\newcommand{\vw}{\bm{w}}
\newcommand{\vx}{\bm{x}}
\newcommand{\vy}{\bm{y}}
\newcommand{\vz}{\bm{z}}

\newcommand{\Xgood}{X_{\mathsf{good}}}
\newcommand{\Xbad}{X_{\mathsf{bad}}}
\newcommand{\Xhat}{\widehat{X}}
\newcommand{\hhat}{\widehat{h}}
\newcommand{\hstar}{h^{\star}}
\newcommand{\Vhat}{\widehat{V}}
\newcommand{\Sigmahat}{\widehat{\Sigma}}

\newcommand{\pinv}[1]{#1^{+}}
\newcommand{\ppinv}[1]{\inparen{#1}^{+}}

\DeclareRobustCommand{\mybox}[2][gray!20]{%
\begin{tcolorbox}[   %% Adjust the following parameters at will.
        % breakable,
        left=0pt,
        right=0pt,
        top=0pt,
        bottom=0pt,
        colback=#1,
        colframe=#1,
        width=\dimexpr\textwidth\relax, 
        enlarge left by=0mm,
        boxsep=5pt,
        arc=0pt,outer arc=0pt,
        parbox=false,
        ]
        #2
\end{tcolorbox}
}

\usepackage{multirow}
\usepackage{soul}

\usepackage{tikz}

\tcbuselibrary{listings,breakable}

\definecolor{asparagus}{rgb}{0.53, 0.66, 0.42}
\definecolor{sacramentostategreen}{rgb}{0.0, 0.3, 0.15}
\definecolor{teal}{rgb}{0.0, 0.5, 0.5}
\definecolor{extresults}{rgb}{0.86, 0.86, 0.50}
\definecolor{defn}{rgb}{0.94, 0.63, 0.94}
\definecolor{forestgreen}{rgb}{0.13, 0.6, 0.13}

\newcommand{\protocol}[3]{
    \stepcounter{figure}
    \vspace{0.15cm}
    { \small
    \begin{tcolorbox}[breakable, colback=#3!12]
    \begin{center}
    {\bf \underline{#1}}
    \end{center}
    
    #2
    \end{tcolorbox}
    }
}

\newcommand{\nnote}[1]{ $\ll$\textsf{\color{blue} Naren: { #1}}$\gg$}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newenvironment{cbox}[2]% environment name
{% begin code
  \begin{tcolorbox}[
  enhanced,
  breakable,
  colback=#1!5!white,
  colframe=#1!75!black,
  left=0pt,right=0pt,top=0pt,bottom=0pt,
  title={\centering #2}]
}%
{% end code
  \end{tcolorbox}\ignorespacesafterend
}

\newenvironment{cdashbox}[1]% environment name
{% begin code
  \begin{tcolorbox}[
  enhanced,
breakable,
colframe=#1!50!white,
colback=#1!5!white,
colbacktitle=green!15!white,
coltitle=green!50!black,
borderline={0.5mm}{0mm}{#1!15!white},
borderline={0.5mm}{0mm}{#1!50!white,dashed},
  left=0pt,right=0pt,top=0pt,bottom=0pt,
  ]
}%
{% end code
  \end{tcolorbox}\ignorespacesafterend
}
